Vision Language Models are Biased

Large language models (LLMs) memorize a vast amount of prior knowledge from the Internet that helps them on downstream tasks but also may notoriously sway their outputs towards wrong or biased answers. In this work, we test how the knowledge about popular subjects hurt the accuracy of vision language models (VLMs) on standard, objective visual tasks of counting and identification. We find that state-of-the-art VLMs are strongly biased (e.g., unable to recognize the 4th stripe has been added to a 3-stripe Adidas logo) scoring an average of 17.05% accuracy in counting (e.g., counting stripes in an Adidas-like logo) across 7 diverse domains from animals, logos, chess, board games, optical illusions, to patterned grids. Removing image backgrounds nearly doubles accuracy (21.09 percentage points), revealing that contextual visual cues trigger these biased responses. Further analysis of VLMs' reasoning patterns shows that counting accuracy initially rises with thinking tokens, reaching ~40%, before declining with excessive reasoning. Our work presents an interesting failure mode in VLMs and a human-supervised automated framework for testing VLM biases. Code and data are available at: vlmsarebiased.github.io.

==> tables_and_figures/bias_error_vs_sanity_check.tex <==
% Remove any figure environment and use a plain layout
\noindent
\begin{minipage}[t]{0.45\textwidth}
\vspace{-0.75}
  \captionof{table}{All VLMs achieve 100\% on identification and counting tasks, showing full recognition of original images in ViasTest.}
  \vspace{0.5em}
  \centering
  \begin{tabular}{@{}lcc@{}}
    \toprule
    Model & ID & Count \\
    \midrule
    Gemini-2.5 Pro & 100.00 & 100.00 \\
    Sonnet-3.7 & 100.00 & 100.00 \\
    GPT-4.1 & 100.00 & 100.00 \\
    o3 & 100.00 & 100.00 \\
    o4-mini & 100.00 & 100.00 \\
    \bottomrule
  \end{tabular}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.52\textwidth}
  \centering
  \includegraphics[width=\textwidth]{images/task_mean_performance.pdf}
  \captionof{figure}{Across all tasks, VLMs average \textbf{\textcolor{blue}{17.05\%}} correct, \textbf{\textcolor{orange}{75.70\%}} bias-aligned errors, and \textbf{\textcolor{red}{7.25\%}} other errors.}
\end{minipage}

==> tables_and_figures/fig_bias_error.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{images/task_mean_performance.pdf}
    \caption{Across all tasks, VLMs average  {\sethlcolor{RoyalBlue}\hl{\textbf{17.05\%}}} correct, {\sethlcolor{YellowOrange}\hl{\textbf{75.70\%}}} bias-aligned errors, and {\sethlcolor{Salmon}\hl{\textbf{7.25\%}}} other errors, indicating that these models overwhelmingly default to learned expectations instead of actual visual reasoning.}
    \label{fig:bias-errors}
\end{figure}

==> tables_and_figures/fig_logos_examples.tex <==
% =============================================
\begin{figure}[ht]
\centering
\small
\begin{AIbox}{Logos}
\centering


    \begin{tabular}{lp{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c}
    &\multicolumn{2}{c}{\makecell{\textbf{(a) Adidas}}} 
    &\multicolumn{2}{c}{\makecell{\textbf{(b) Mercedes}}}
    &\multicolumn{2}{c}{\makecell{\textbf{(c) Audi}}}
    &\multicolumn{2}{c}{\makecell{\textbf{(d) Adidas}}} 
    &\multicolumn{2}{c}{\makecell{\textbf{(e) Nike}}}
    \\
     &\multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/adidas-red-running-5_1152.png}}
     &\multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/mercedes_benz-white-convertible_1152.png}}
     &\multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/audi-black-convertible_1152.png}}
     &\multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/adidas-white-tennis-1_1152.png}}
     &\multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/nike-white-basketball-1_1152.png}}
     \\ 
     % Gemini 2.5


% Gemini 2.5
\rowcolor{lightgray}
\raisebox{-0.2\height}\geminilogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} \\ 


% Sonnet 3.7
\raisebox{-0.2\height}\newsonnetlogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% GPT-4.1
\rowcolor{lightgray}
\raisebox{-0.2\height}\gptfourlogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% GPT-o3
\raisebox{-0.2\height}\gptfulllogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% GPT-o4-mini
\rowcolor{lightgray}
\raisebox{-0.2\height}\gptminilogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 



     \end{tabular}
    \vspace{4pt}
    \centering
    \begin{tabular}{cccccccccccccc}
     \raisebox{-0.1\height}\geminilogo~\gemini 
     & \raisebox{-0.1\height}\newsonnetlogo~\newsonnet 
     & \raisebox{-0.1\height}\gptfourlogo~\gptfour 
     & \raisebox{-0.1\height}\gptfulllogo~\gptfull 
     & \raisebox{-0.1\height}\gptminilogo~\gptmini
     \\
    \end{tabular}
     \hfill \break
    \hfill \break
    \raggedright
      
\end{AIbox}
\caption{}
\label{appfig:circled_word_prompt1}
\end{figure}
% =============================================

==> tables_and_figures/fig_patterned_grid_examples.tex <==
% =============================================
\begin{figure}[ht]
\centering
\small
\begin{AIbox}{Abstract Images: Patterned Grid}
\centering


    \begin{tabular}{lp{0.8cm}c|p{0.8cm}c|p{0.8cm}c|p{0.8cm}c}
    &\multicolumn{2}{c}{\makecell{\textbf{(a) Dice}\\Remove}}
    &\multicolumn{2}{c}{\makecell{\textbf{(b) Dice}\\Replace}}
    &\multicolumn{2}{c}{\makecell{\textbf{(c) Tally}\\Remove}}
    &\multicolumn{2}{c}{\makecell{\textbf{(d) Tally}\\Add}} 

    \\
    
     &\multicolumn{2}{c}{\includegraphics[width=0.2\textwidth]{images/patterned_grid_examples/dice_001_remove_C3_notitle_px1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.2\textwidth]{images/patterned_grid_examples/dice_001_replace_C3_notitle_px1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.2\textwidth]{images/patterned_grid_examples/tally_001_remove_C3_notitle_px1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.2\textwidth]{images/patterned_grid_examples/tally_001_add_C3_notitle_px1152.png}}
     \\ 


% Gemini 2.5
\rowcolor{lightgray}
\raisebox{-0.2\height}\geminilogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 3
& \textcolor{red}{\xmark} \\ 


% Sonnet 3.7
\raisebox{-0.2\height}\newsonnetlogo & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} \\ 


% GPT-4.1
\rowcolor{lightgray}
\raisebox{-0.2\height}\gptfourlogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} \\ 


% GPT-o3
\raisebox{-0.2\height}\gptfulllogo & \centering 3
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} \\ 


% GPT-o4-mini
\rowcolor{lightgray}
\raisebox{-0.2\height}\gptminilogo & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 3
& \textcolor{red}{\xmark} \\ 

\midrule
% Expected Bias
\textbf{Bias} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} \\ 


% Ground Truth
\rowcolor{lightgray}
\textbf{GT} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} \\ 

     \end{tabular}
    \vspace{4pt}
    \centering
    \begin{tabular}{cccccccccccccc}
     \raisebox{-0.1\height}\geminilogo~\gemini 
     & \raisebox{-0.1\height}\newsonnetlogo~\newsonnet 
     & \raisebox{-0.1\height}\gptfourlogo~\gptfour 
     & \raisebox{-0.1\height}\gptfulllogo~\gptfull 
     & \raisebox{-0.1\height}\gptminilogo~\gptmini
     \\
    \end{tabular}
     \hfill \break
    \hfill \break
    \raggedright
    \scriptsize
      \textbf{(a), (b):} How many \textbf{circles} are there in cell \textbf{C3}? Answer with a number in curly brackets, e.g., \{9\}. \\
      \textbf{(c), (d):} How many \textbf{lines} are there in cell \textbf{C3}? Answer with a number in curly brackets, e.g., \{9\}. \\
      
\end{AIbox}
\caption{All VLMs, except \newsonnetlogo~\newsonnet, fail to correctly identify the abnormal cell (C3) in both the \patternedgridicon~patterned grids.}
\label{fig:patterned_grid}
\end{figure}
% =============================================

==> tables_and_figures/fig_real_world.tex <==
% =============================================
\begin{figure}[ht]
\begin{AIbox}{Real-world images: Animals and Logos}
    \raggedright
\scriptsize
      \animalicon~\textbf{(a), (b):} How many \textbf{legs} does this animal have? Answer with a number in curly brackets, e.g., \{9\}. \\
      \logoicon~\textbf{(c):} How many visible \textbf{stripes} are there on the logo of the left shoe? Answer with a number in curly brackets, e.g., \{9\}. \\
      \logoicon~\textbf{(d):} How many \textbf{points} on the star are there in the logo of this car? Answer with a number in curly brackets, e.g., \{9\}. \\
      \logoicon~\textbf{(e):} How many visible \textbf{black stylized curves} are there in the logo of the left shoe?
    \hfill \break
    \hfill \break
\footnotesize
\centering
    \begin{tabular}{lp{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c}
    &\multicolumn{2}{c}{\makecell{\textbf{(a) Elephant}}} 
    &\multicolumn{2}{c}{\makecell{\textbf{(b) Chicken}}}
    &\multicolumn{2}{c}{\makecell{\textbf{(c) Adidas}}}
    &\multicolumn{2}{c}{\makecell{\textbf{(d) Mercedes}}} 
    &\multicolumn{2}{c}{\makecell{\textbf{(e) Nike}}}
    \\
     &\multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/animal_examples/african elephant_2_0_1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/animal_examples/chicken_0_3_1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/adidas-red-running-5_1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/mercedes_benz-white-convertible_1152.png}}
     & \multicolumn{2}{c}{\includegraphics[width=0.15\textwidth]{images/logo_examples/nike-white-basketball-1_1152.png}} 
     \\ 
     % Gemini 2.5
% Gemini 2.5
\rowcolor{lightgray}
\raisebox{-0.2\height}\geminilogo & \centering 4
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} \\ 


% Sonnet 3.7
\raisebox{-0.2\height}\newsonnetlogo & \centering 4
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% GPT-4.1
\rowcolor{lightgray}
\raisebox{-0.2\height}\gptfourlogo & \centering 6
& \textcolor{red}{\xmark} & \centering 4
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% GPT-o3
\raisebox{-0.2\height}\gptfulllogo & \centering 4
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% GPT-o4-mini
\rowcolor{lightgray}
\raisebox{-0.2\height}\gptminilogo & \centering 4
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 

\midrule

% Expected Bias
\textbf{Bias} & \centering 4
& \textcolor{red}{\xmark} & \centering 2
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 1
& \textcolor{red}{\xmark} \\ 


% Ground Truth
\rowcolor{lightgray}
\textbf{GT} & \centering 5
& \textcolor{ForestGreen}{\cmark} & \centering 3
& \textcolor{ForestGreen}{\cmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} \\ 

     \end{tabular}
    \vspace{4pt}
    \centering
    \begin{tabular}{cccccccccccccc}
     \raisebox{-0.1\height}\geminilogo~\gemini 
     & \raisebox{-0.1\height}\newsonnetlogo~\newsonnet 
     & \raisebox{-0.1\height}\gptfourlogo~\gptfour 
     & \raisebox{-0.1\height}\gptfulllogo~\gptfull 
     & \raisebox{-0.1\height}\gptminilogo~\gptmini
     \\
    \end{tabular}

      
\end{AIbox}
\caption{VLMs often fail to detect subtle visual details across real-world images of \animalicon~animals and \logoicon~logos. They frequently provide incorrect answers on tasks involving modified object properties (\eg, leg counts, logo stripes, star points, or curve shapes). These errors reveal a lack of sensitivity to small but meaningful modifications in real-world images.}
\label{fig:real-world}
\end{figure}
% =============================================

==> tables_and_figures/full_examples.tex <==
% ---------------------
\begin{figure}[h]

\begin{AIbox}{Examples of VLM failures across 7 domains of \biastest}
    % \hspace{-0.04\textwidth}
        \footnotesize
        \raggedright
      \animalicon~How many \textbf{legs} does this animal have? Answer with a number in curly brackets, e.g., \{9\}. \\
      \logoicon~How many \textbf{points} are there on the star in the logo of this car? Answer with a number in curly brackets, e.g., \{9\}. \\
      \flagicon~How many \textbf{stripes} are there in this flag? Answer with a number in curly brackets, e.g., \{9\}. \\
      \chessicon~How many \textbf{chess pieces} are there on this board? Answer with a number in curly brackets, e.g., \{9\}. \\
      \boardgameicon~How many \textbf{rows} are there on this board?  Answer with a number in curly brackets, e.g., \{9\}. \\
      \illusionicon~Are the two horizontal lines \textbf{parallel}? Answer in curly brackets, e.g., \{Yes\} or \{No\}. \\
      \patternedgridicon~How many \textbf{circles} are there in cell C3? Answer with a number in curly brackets, e.g., \{9\}. 
        \hfill \break
    \hfill \break
    \centering
    \begin{tabular}{lp{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.3cm}c|p{0.2cm}c}
    
    &\multicolumn{2}{c}{a. \textbf{\animalicon}}
    &\multicolumn{2}{c}{b. \textbf{\logoicon}}
    &\multicolumn{2}{c}{c. \textbf{\flagicon}}
    &\multicolumn{2}{c}{d. \textbf{\chessicon}}
    &\multicolumn{2}{c}{e. \textbf{\boardgameicon}}
    &\multicolumn{2}{c}{f. \textbf{\illusionicon}}
    &\multicolumn{2}{c}{g. \textbf{\patternedgridicon}}\\
    
     &\multicolumn{2}{c}{\includegraphics[width=0.06\textwidth]{images/animal_examples/chicken_0_3_1152.png}} 
     & \multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/logo_examples/mercedes_benz-white-convertible_1152.png}} 
     &\multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/full_examples/us_14_stripes.png}} 
     &\multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/full_examples/chess_remove_piece.png}} 
     &\multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/full_examples/sudoku_8_rows.png}}
     &\multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/full_examples/zonner_illusion_fake.png}}
     &\multicolumn{2}{c}{\includegraphics[width=0.10\textwidth]{images/full_examples/dice_C3.png}}
     
    \\ 
     \rowcolor{lightgray}
     \raisebox{-0.2\height}\geminilogo 
     & \centering 2
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     & \centering 13
     & \textcolor{red}{\xmark}
     & \centering 32
     & \textcolor{red}{\xmark}
     & \centering 9
     & \textcolor{red}{\xmark}
     & \centering Yes
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     \\ 
     
     \raisebox{-0.2\height}\newsonnetlogo 
     & \centering 2
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     & \centering 13
     & \textcolor{red}{\xmark}
     & \centering 32
     & \textcolor{red}{\xmark}
     & \centering 9
     &\textcolor{red}{\xmark}
     & \centering No
     & \textcolor{ForestGreen}{\cmark} 
     & \centering 2
     & \textcolor{ForestGreen}{\cmark} 
     \\ 
     
     \rowcolor{lightgray}
     \raisebox{-0.2\height}\gptfourlogo 
     & \centering 4
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     & \centering 13
     & \textcolor{red}{\xmark}
     & \centering 32
     & \textcolor{red}{\xmark}
     & \centering 9
     & \textcolor{red}{\xmark}
     & \centering Yes
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     \\ 
     
     \raisebox{-0.2\height}\gptfulllogo 
      & \centering 2
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
      & \centering 13
     & \textcolor{red}{\xmark}
     & \centering 32
     & \textcolor{red}{\xmark}
     & \centering 9
     & \textcolor{red}{\xmark}
     & \centering Yes
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     \\ 

     \rowcolor{lightgray}
     \raisebox{-0.2\height}\gptminilogo 
     & \centering 2
     & \textcolor{red}{\xmark}
    & \centering 3
     & \textcolor{red}{\xmark}
     & \centering 13
     & \textcolor{red}{\xmark}
     & \centering 32
     & \textcolor{red}{\xmark}
     & \centering 9
     & \textcolor{red}{\xmark}
     & \centering Yes
     & \textcolor{red}{\xmark}
     & \centering 3
     & \textcolor{red}{\xmark}
     \\ 

     \midrule
% Expected Bias
{Bias} & \centering 2
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} & \centering 13
& \textcolor{red}{\xmark} & \centering 32
& \textcolor{red}{\xmark} & \centering 9
& \textcolor{red}{\xmark} & \centering Yes
& \textcolor{red}{\xmark} & \centering 3
& \textcolor{red}{\xmark} \\ 


% Ground Truth
\rowcolor{lightgray}
{GT} & \centering 3
& \textcolor{ForestGreen}{\cmark} & \centering 4
& \textcolor{ForestGreen}{\cmark} & \centering 14
& \textcolor{ForestGreen}{\cmark} & \centering 31
& \textcolor{ForestGreen}{\cmark} & \centering 10
& \textcolor{ForestGreen}{\cmark} & \centering No
& \textcolor{ForestGreen}{\cmark} & \centering 2
& \textcolor{ForestGreen}{\cmark} \\ 
     \end{tabular}
    \vspace{4pt}
    \centering
    \begin{tabular}{cccccccccccccc}
     \raisebox{-0.1\height}\geminilogo~\geminifull
     & \raisebox{-0.1\height}\newsonnetlogo~\newsonnet 
     & \raisebox{-0.1\height}\gptfourlogo~\gptfour 
     & \raisebox{-0.1\height}\gptfulllogo~\gptfull 
     & \raisebox{-0.1\height}\gptminilogo~\gptmini
     \\
      \end{tabular}
    
\end{AIbox}
\caption{VLMs fail on 6 counting tasks (a--e \& g) and one low-level vision task (f).
% simple visual reasoning tasks in \biastest, including basic counting, pattern recognition, and comparison.
}
\label{fig:teaser}
\end{figure}
%------------------------------------------------

==> tables_and_figures/helpful_prompt.tex <==
\begin{wraptable}{r}{0.53\textwidth} 
\caption{Task mean accuracy (\%) under different prompting conditions. While adversarial prompts (\ie, in-image titles; $\Delta$=\decreasenoparent{4.49}) and helpful strategies (\ie, Debiased Prompt, Double-Check; mean $\Delta$=\increasenoparent{2.29}) influence performance to some extent, they do not resolve the core issue of visual bias
% The In-Image Title setting significantly decreases performance \decrease{4.49\%}, suggesting that visual priming with object names reinforces prior biases. In contrast, the Yes/No Format yields the highest mean accuracy \increase {8.06\%}, though this likely reflects the simplicity of binary response rather than improved visual reasoning. Helpful prompting strategies, such as Debiased Prompt \increase{1.87\%} and Double-Check \increase{2.70\%} offer consistent but modest improvements, indicating their potential to support more reliable model behavior.
}
\centering
\resizebox{0.53\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Model
  & Baseline
  & \multicolumn{1}{c}{Adversarial}
  & \multicolumn{2}{c}{Helpful textual prompt} \\
\cmidrule(lr){3-3}\cmidrule(lr){4-5}
  &  
  & w/ In-image Title
  % & Y/N 
  & w/ Debiased Prompt
  & w/ Double-Check
\\
\midrule
\geminilogo~\geminifull 
& 16.02 
& 12.04 \decrease{3.98}
% & 20.63 \increase{4.61} 
& 19.72 \increase{3.70} 
& 20.22 \increase{4.20}
 \\
\newsonnetlogo~\newsonnet 
& 16.59 
& 13.78 \decrease{2.81} 
% & 23.08 \increase{6.49} 
& 19.29 \increase{2.70}
& 20.86 \increase{4.27}
\\

\gptfourlogo~\gptfour 
& 13.88 
& 11.21 \decrease{2.67} 
% & 26.10 \increase{12.22} 
& 14.38 \increase{0.50} 
& 16.00 \increase{2.12}

\\
\gptfulllogo~\gptfull 
& 18.50 
& 12.09 \decrease{6.41} 
% & 26.15 \increase{7.65} 
& 18.94 \increase{0.44} 
& 21.02 \increase{2.52} \\
\gptminilogo~\gptmini 
& 20.25 
& 13.69 \decrease{6.56} 
% & 29.61 \increase{9.36} 
& 22.25 \increase{2.00} 
& 20.61 \increase{0.36} \\
\midrule
% \rowcolor{lightgray}
Mean 
& 17.05 
& 12.56 \decrease{4.49} 
% & 25.11 \increase{8.06} 
& 18.92 \increase{1.87}
& 19.75 \increase{2.70} \\
\bottomrule
\end{tabular}
}
  \vspace{-0.3in}
\label{tab:prompt_results}
\end{wraptable}


==> tables_and_figures/sanity_check.tex <==
\begin{wraptable}{r}{0.35\textwidth}
\vspace{-0.15in}
\caption{All VLMs achieve 100\% on identification and counting tasks, showing that they fully recognize and understand the original version of modified images in \viastest
% This confirms that subsequent failures on modified samples are not due to the lack of familiarity or visual grounding, but because they fail to notice the subtle changes.
}
\small
\centering
\setlength{\tabcolsep}{0.2pt}
\begin{tabular}{lccc}
\toprule
Model & ID & Counting \\
\midrule
\raisebox{-.2\height}\geminilogo~\geminifull~~~  & 100.00 & 100.00 \\
\raisebox{-.2\height}\newsonnetlogo~\newsonnet~~~ & 100.00 & 100.00 \\
\raisebox{-.2\height}\gptfourlogo~\gptfour~~~  & 100.00 & 100.00 \\
\raisebox{-.2\height}\gptfulllogo~\gptfull~~~   & 100.00 & 100.00 \\
\raisebox{-.2\height}\gptminilogo~\gptmini~~~  & 100.00 & 100.00 \\
% \rowcolor{lightgray}
\bottomrule
\end{tabular}
\label{tab:sanity-check}

\end{wraptable}


==> tables_and_figures/tab_animal.tex <==
\begin{table}[h]
\caption{In \animalicon~animal task, VLMs perform poorly when estimating the correct number of legs for birds (2 legs) and mammals (4 legs). Even the best-performing model, \gptfourlogo~\gptfour, achieves only \textbf{9.52\%}. The overall \hallucinatepanel{mean accuracy} across all models is just \hallucinatepanel{2.12\%}, indicating that current VLMs almost entirely fail to handle basic animal attribute reasoning under subtle visual changes.}
\centering
\begin{tabular}{lcccc}
\toprule
Model & \makecell{Bird\\(2 legs)} & \makecell{Mammals\\(4 legs)} & Mean \\
\midrule
\geminilogo~\geminifull 
& 0.00
& 0.00
& 0.00
\\
\newsonnetlogo~\newsonnet 
& 0.00
& 0.00
& 0.00
\\
\gptfourlogo~\gptfour 
& \textbf{5.07}
& \textbf{11.03}
& \textbf{9.52}
\\
\gptfulllogo~\gptfull 
& 0.00
& 1.23
& 0.92
\\
\gptminilogo~\gptmini 
& 0.00
& 0.25
& 0.18 
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 1.01
& 2.50
& \hallucinatepanel{2.12}
\\
\bottomrule
\end{tabular}
\label{tab:results_animal}
\end{table}

==> tables_and_figures/tab_chess_pieces.tex <==
\begin{table}[h]
\caption{Thinking models (\ie, \geminilogo~\geminifull, \gptfulllogo~\gptfull, and \gptminilogo~\gptmini) outperform others on \chessicon~the chess and xiangqi piece modification task, indicating that models with reasoning capabilities may be better at carefully examining the board to detect abnormalities, compared to non-thinking models (\ie, \newsonnetlogo~\newsonnet, \gptfourlogo~\gptfour)}
\centering
\begin{tabular}{lcccccccc}
\toprule
Model
  & Chess
  & Xiangqi
  & Mean \\
\midrule
\geminilogo~\geminifull 
& 17.36
& \textbf{36.11}
& 26.74
\\
\newsonnetlogo~\newsonnet 
& 7.64
& 10.42
& 9.03
\\
\gptfourlogo~\gptfour 
& 11.81
& 5.56
& 8.68
\\
\gptfulllogo~\gptfull 
& \textbf{56.94}
& 28.47
& 42.71
\\
\gptminilogo~\gptmini 
& 55.56
& 32.64
& \textbf{44.10}
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 29.86
& 22.64
& \hallucinatepanel{26.25}

\\
\bottomrule
\end{tabular}
\label{tab:chess_pieces_results}
\end{table}


% \begin{table}[h]
% \caption{Thinking models (\ie, \geminilogo~\geminifull, \gptfulllogo~\gptfull, and \gptminilogo~\gptmini) outperform others on \chessicon~the chess and xiangqi piece modification task, indicating that models with reasoning capabilities may be better at carefully examining the board to detect abnormalities, compared to non-thinking models (\ie, \newsonnetlogo~\newsonnet, \gptfourlogo~\gptfour)}
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% Model
%   & \multicolumn{2}{c}{Chess}
%   & \multicolumn{2}{c}{Xiangqi}
%   & Mean \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%   & Remove
%   & Replace
%   & Remove
%   & Replace
%   &  \\
% \midrule
% \geminilogo~\geminifull 
% & 16.67
% & 18.06
% & \textbf{51.39}
% & 20.83
% & 26.74
% \\
% \newsonnetlogo~\newsonnet 
% & 5.56
% & 9.72
% & 6.94
% & 13.89
% & 9.03
% \\
% \gptfourlogo~\gptfour 
% & 0.00
% & 23.61
% & 5.56
% & 5.56
% & 8.68
% \\
% \gptfulllogo~\gptfull 
% & \textbf{38.89}
% & 75.00
% & 33.33
% & 23.61
% & 42.71
% \\
% \gptminilogo~\gptmini 
% & 23.61
% & \textbf{87.50}
% & 31.94
% & \textbf{33.33}
% & \textbf{44.10}
% \\
% \midrule
% % \rowcolor{lightgray}
% Mean 
% & 16.94
% & 42.78
% & 25.83
% & 19.44
% & \hallucinatepanel{26.25}

% \\
% \bottomrule
% \end{tabular}
% \label{tab:model_performance}
% \end{table}

==> tables_and_figures/tab_flag.tex <==


\begin{table}[h]
\caption{VLMs perform better on star modifications (11.79\%) than on stripe changes (4.52\%) in the \flagicon~national flag task. These results suggest that VLMs are more sensitive to object-level changes (e.g., missing stars) than to subtle structural changes (\eg, extra stripes).}
\centering
\begin{tabular}{lcccc}
\toprule
Model
  & Stars
  & Stripes
  & Mean \\
\midrule
\geminilogo~\geminifull 
& 11.54
& \textbf{8.33}
& 10.42
\\
\newsonnetlogo~\newsonnet 
& \textbf{20.51}
& 1.19
& 13.75
\\
\gptfourlogo~\gptfour 
& 3.21
& 1.19
& 2.50
\\
\gptfulllogo~\gptfull 
& 5.13
& 4.76
& 5.00
\\
\gptminilogo~\gptmini 
& 18.59
& 7.14
& \textbf{14.58}
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 11.79
& 4.52
& \hallucinatepanel{9.25}

\\
\bottomrule
\end{tabular}
\label{tab:flag_results}
\end{table}

% \begin{table}[h]
% \caption{VLMs perform better on star modifications (11.79\%) than on stripe changes (4.52\%) in the \flagicon~national flag task. These results suggest that VLMs are more sensitive to object-level changes (e.g., missing stars) than to subtle structural changes (\eg, extra stripes).}
% \centering
% \begin{tabular}{lccccccc}
% \toprule
% Model
%   & \multicolumn{2}{c}{Star}
%   & \multicolumn{2}{c}{Stripe}
%   & Mean \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%   & Add
%   & Remove
%   & Add
%   & Remove
%   &  \\
% \midrule
% \geminilogo~\geminifull 
% & 16.67
% & 6.41
% & \textbf{2.38}
% & \textbf{14.29}
% & 10.42
% \\
% \newsonnetlogo~\newsonnet 
% & \textbf{19.23}
% & \textbf{21.79}
% & 0.00
% & 2.38
% & 13.75
% \\
% \gptfourlogo~\gptfour 
% & 2.56
% & 3.85
% & 0.00
% & 2.38
% & 2.50
% \\
% \gptfulllogo~\gptfull 
% & 2.56
% & 7.69
% & \textbf{2.38}
% & 7.14
% & 5.00
% \\
% \gptminilogo~\gptmini 
% & 17.95
% & 19.23
% & \textbf{2.38}
% & 11.90
% & \textbf{14.58}
% \\
% \midrule
% % \rowcolor{lightgray}
% Mean 
% & 11.79
% & 11.79
% & 1.43
% & 7.62
% & \hallucinatepanel{9.25}

% \\
% \bottomrule
% \end{tabular}
% \label{tab:model_performance}
% \end{table}

==> tables_and_figures/tab_illusion_grid.tex <==
\begin{table}[h]
\caption{No VLM performs well on both original and modified \illusionicon~optical illusions, highlighting a fundamental trade-off. Interestingly, \newsonnetlogo~\newsonnet achieves the highest overall mean accuracy (\textbf{54.29\%}) and performs best on modified illusions (\textbf{65.91\%}), but is the worst on original ones (42.68\%). This show \newsonnetlogo~\newsonnet occasionally exhibits human-like perceptual bias, aligning more closely with how humans perceive the original illusions. 
% These results suggest that training VLMs to handle both canonical illusions and their visually corrected versions may be inherently challenging due to competing perceptual versus knowledge-driven biases.
}
\centering
\begin{tabular}{lcccc}
\toprule
Model & Original & Modified & Mean \\
\midrule
\geminilogo~\geminifull 
& 73.16
& 26.52
& 49.81
\\
\newsonnetlogo~\newsonnet 
& 42.68
& \textbf{65.91}
& \textbf{54.29}
\\
\gptfourlogo~\gptfour 
& \textbf{92.17}
& 5.05
& 48.61
\\
\gptfulllogo~\gptfull 
& 91.67
& 9.09
& 50.38
\\
\gptminilogo~\gptmini 
& 90.40
& 12.12
& 51.26
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 78.02
& 23.74
& \hallucinatepanel{50.87}
\\
\bottomrule
\end{tabular}
\label{tab:illusion_results}
\end{table}

==> tables_and_figures/tab_logos.tex <==
\begin{table}[h]
\caption{VLMs show limited ability to detect logo modifications, with a \hallucinatepanel{mean accuracy} of only \hallucinatepanel{6.13\%}. Notably, all \logoicon~logos appear in their correct real-world contexts (e.g., modified Nike logo on Nike shoes). This low \hallucinatepanel{mean accuracy} suggests that models rely heavily on prior knowledge and context cues, leading to overconfident predictions even when clearly altered visual details.}
\centering
\begin{tabular}{lccccc}
\toprule
Model & Shoe Logos &Car Logos & Mean \\
\midrule
\geminilogo~\geminifull 
& 5.80
& 0.00
& 1.96
\\
\newsonnetlogo~\newsonnet 
& 8.15
& 0.00
& 2.72
\\
\gptfourlogo~\gptfour 
& \textbf{25.36}
& \textbf{1.11}
& 9.07
\\
\gptfulllogo~\gptfull 
& 21.01
& \textbf{1.11}
& 7.60
\\
\gptminilogo~\gptmini 
& 27.54
& 0.00
& \textbf{9.31}
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 17.57
& 0.44
& \hallucinatepanel{6.13}

\\
\bottomrule
\end{tabular}
\label{tab:logo_results}
\end{table}

% \begin{table}[h]
% \caption{VLMs show limited ability to detect logo modifications, with a \hallucinatepanel{mean accuracy} of only \hallucinatepanel{6.13\%}. Notably, all \logoicon~logos appear in their correct real-world contexts (e.g., modified Nike logo on Nike shoes). Performance is relatively higher on Nike logos (31.95\%), yet still far from perfect, despite the modification involving only a simple addition of one stylized curve. This suggests that models rely heavily on prior knowledge and context cues, leading to overconfident predictions even when clearly altered visual details.}
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% Model & \multicolumn{2}{c}{Shoe Logos} & \multicolumn{3}{c}{Car Logos} & Mean \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-6}
% & Nike & Adidas & Audi & Maserati & Mercedes & \\
% \midrule
% \geminilogo~\geminifull 
% & 10.61
% & 1.39
% & 0.00
% & 0.00
% & 0.00
% & 1.96
% \\
% \newsonnetlogo~\newsonnet 
% & 14.29
% & 2.78
% & 0.00
% & 0.00
% & 0.00
% & 2.72
% \\
% \gptfourlogo~\gptfour 
% & \textbf{53.03}
% & 0.00
% & 0.00
% & \textbf{2.22}
% & 0.00
% & 9.07
% \\
% \gptfulllogo~\gptfull 
% & 31.82
% & \textbf{11.11}
% & 0.00
% & \textbf{2.22}
% & 0.00
% & 7.60
% \\
% \gptminilogo~\gptmini 
% & 50.00
% & 6.94
% & 0.00
% & 0.00
% & 0.00
% & \textbf{9.31}
% \\
% \midrule
% % \rowcolor{lightgray}
% Mean 
% & 31.95
% & 4.44
% & 0.00
% & 0.89
% & 0.00
% & \hallucinatepanel{6.13}

% \\
% \bottomrule
% \end{tabular}
% \label{tab:model_performance}
% \end{table}

==> tables_and_figures/tab_merged_animal_logos_flag.tex <==
\begin{table}[h]
\caption{Performance comparison of VLMs across three visual reasoning tasks with subtle visual modifications. All tasks show poor performance, with mean accuracies of 2.12\% (Animal), 6.13\% (Logo), and 9.25\% (Flag).}
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l ccc c ccc c ccc}
\toprule
& \multicolumn{3}{c}{Task 1: \animalicon~Animal} & & \multicolumn{3}{c}{Task 2: \logoicon~Logo} & & \multicolumn{3}{c}{Task 3: \flagicon~Flag} \\
\cmidrule(lr){2-4} \cmidrule(lr){6-8} \cmidrule(lr){10-12}
Model & Birds & Mammals & Mean & & Shoes & Cars & Mean & & Stars & Stripes & Mean \\
\midrule
\geminilogo~\geminifull 
& 0.00 & 0.00 & 0.00 & & 5.80 & 0.00 & 1.96 & & 11.54 & \textbf{8.33} & 10.42 \\
\newsonnetlogo~\newsonnet 
& 0.00 & 0.00 & 0.00 & & 8.15 & 0.00 & 2.72 & & \textbf{20.51} & 1.19 & 13.75 \\
\gptfourlogo~\gptfour 
& \textbf{5.07} & \textbf{11.03} & \textbf{9.52} & & \textbf{25.36} & \textbf{1.11} & 9.07 & & 3.21 & 1.19 & 2.50 \\
\gptfulllogo~\gptfull 
& 0.00 & 1.23 & 0.92 & & 21.01 & \textbf{1.11} & 7.60 & & 5.13 & 4.76 & 5.00 \\
\gptminilogo~\gptmini 
& 0.00 & 0.25 & 0.18 & & 27.54 & 0.00 & \textbf{9.31} & & 18.59 & 7.14 & \textbf{14.58} \\
\midrule
Mean & 1.01 & 2.50 & \hallucinatepanel{2.12} & & 17.57 & 0.44 & \hallucinatepanel{6.13} & & 11.79 & 4.52 & \hallucinatepanel{9.25} \\
\bottomrule
\end{tabular}
\label{tab:combined_results}
\end{table}

==> tables_and_figures/tab_patterned_grid.tex <==
\begin{table}[h]
\caption{VLMs struggle more with detecting modifications in \patternedgridicon~patterned grid task that preserve the structure of the cell (\ie, removal; 17.26\%) than those that visibly disrupt it (\ie, replacement/addition; 27.62\%).}
\centering
\begin{tabular}{lccccccc}
\toprule
Model
  & Remove
  & Replace/Add
  & Mean \\
\midrule
\geminilogo~\geminifull 
& 13.10
& 28.57
& 20.83
\\
\newsonnetlogo~\newsonnet 
& \textbf{35.71}
& \textbf{33.33}
& \textbf{34.52}
\\
\gptfourlogo~\gptfour 
& 10.12
& 27.38
& 18.75
\\
\gptfulllogo~\gptfull 
& 14.88
& 26.19
& 20.54
\\
\gptminilogo~\gptmini 
& 12.50
& 22.62
& 17.56
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 17.26
& 27.62
& \hallucinatepanel{22.44}
\\
\bottomrule
\end{tabular}
\label{tab:patterned_grid_results}
\end{table}

% \begin{table}[h]
% \caption{VLMs struggle more with detecting modifications that preserve the structure of the cell (e.g., removal) than those that visibly disrupt it (e.g., replacement or addition). Specifically, accuracy is lower on dice removal (13.81\%) than replacement (18.33\%), and similarly lower on tally removal (20.71\%) compared to tally addition (36.90\%). Even \geminilogo~\geminifull completely fails to detect dice removal (0.00\%). This suggests that subtle changes which maintain visual regularity are harder for VLMs to detect.}
% \centering
% \begin{tabular}{lccccccc}
% \toprule
% Model
%   & \multicolumn{2}{c}{Dice}
%   & \multicolumn{2}{c}{Tally}
%   & Mean \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%   & Remove
%   & Replace
%   & Remove
%   & Add
%   &  \\
% \midrule
% \geminilogo~\geminifull 
% & 0.00
% & 5.95
% & 26.19
% & \textbf{51.19}
% & 20.83
% \\
% \newsonnetlogo~\newsonnet 
% & \textbf{38.10}
% & \textbf{34.52}
% & \textbf{33.33}
% & 32.14
% & \textbf{34.52}
% \\
% \gptfourlogo~\gptfour 
% & 8.33
% & 13.10
% & 11.90
% & 41.67
% & 18.75
% \\
% \gptfulllogo~\gptfull 
% & 9.52
% & 14.29
% & 20.24
% & 38.10
% & 20.54
% \\
% \gptminilogo~\gptmini 
% & 13.10
% & 23.81
% & 11.90
% & 21.43
% & 17.56
% \\
% \midrule
% % \rowcolor{lightgray}
% Mean 
% & 13.81
% & 18.33
% & 20.71
% & 36.90
% & \hallucinatepanel{22.44}
% \\
% \bottomrule
% \end{tabular}
% \label{tab:model_performance}
% \end{table}

==> tables_and_figures/tab_q3.tex <==
\begin{wraptable}{r}{0.53\textwidth} 
\centering
\caption{Accuracy (\%) when VLMs are asked questions that contradict the image (\eg., ``Is this an animal with 4 legs?'' when the image shows 5 legs). VLMs overwhelmingly answer ``Yes'' despite the contradiction, resulting in performance far below the 50\% random baseline on modified images.}
% \scriptsize
\resizebox{0.53\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Model & Original & Modified ($\Delta$) \\
\midrule
\geminilogo~\geminifull 
& 100.00
& 20.63 (\decreasenoparent{79.37})
\\
\newsonnetlogo~\newsonnet 
& 100.00
& 23.08 (\decreasenoparent{76.92})
\\
\gptfourlogo~\gptfour 
& 100.00
& 26.10 (\decreasenoparent{73.90})
\\
\gptfulllogo~\gptfull 
& 100.00
& 26.15 (\decreasenoparent{73.85})
\\
\gptminilogo~\gptmini 
& 100.00
& 29.61 (\decreasenoparent{70.39})
\\
\midrule
% \rowcolor{lightgray}
Mean 
& 100.00
& 25.11 (\decreasenoparent{74.89})
\\
\bottomrule
\vspace{-0.3in}
\end{tabular}
}
\label{tab:modified_original_q3}
\end{wraptable}

==> tables_and_figures/tab_q3_vs_fig_withtitle.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}[t]{0.55\textwidth}
        \centering
        \captionof{table}{Accuracy (\%) when VLMs are asked questions that contradict the image (\eg., ``Is this an animal with 4 legs?'' when the image shows 5 legs). VLMs overwhelmingly answer ``Yes'' despite the contradiction, resulting in performance far below the 50\% random baseline on modified images}
        \resizebox{0.7\textwidth}{!}{
            \begin{tabular}{lccc}
            \toprule
            Model & Original & Modified ($\Delta$) \\
            \midrule
            \geminilogo~\geminifull 
            & 100.00
            & 20.63 (\decreasenoparent{79.37})
            \\
            \newsonnetlogo~\newsonnet 
            & 100.00
            & 23.08 (\decreasenoparent{76.92})
            \\
            \gptfourlogo~\gptfour 
            & 100.00
            & 26.10 (\decreasenoparent{73.90})
            \\
            \gptfulllogo~\gptfull 
            & 100.00
            & 26.15 (\decreasenoparent{73.85})
            \\
            \gptminilogo~\gptmini 
            & 100.00
            & 29.61 (\decreasenoparent{70.39})
            \\
            \midrule
            % \rowcolor{lightgray}
            Mean 
            & 100.00
            & 25.11 (\decreasenoparent{74.89})
            \\
            \bottomrule
            \end{tabular}
        }
        \label{tab:modified_original_q3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.43\textwidth}
    \vspace*{\fill}
        \centering
        \includegraphics[width=0.85\textwidth]{images/illusion_example/illusion_add_title.pdf}
        \captionof{figure}{An example of original vs. modified Ebbinghaus illusion w/ and w/o titles.}
        \label{fig:main_optical_illusion}
    \end{minipage}
\end{figure}
